Robust Decision Trees Against Adversarial Examples

Although adversarial examples and model robustness have been extensively studied in the context of linear models and neural networks, research on this issue in tree-based models and how to make tree-based models robust against adversarial examples is still limited. In this paper, we show that tree based models are also vulnerable to adversarial examples and develop a novel algorithm to learn robust trees. At its core, our method aims to optimize the performance under the worst-case perturbation of input features, which leads to a max-min saddle point problem. Incorporating this saddle point objective into the decision tree building procedure is non-trivial due to the discrete nature of trees --- a naive approach to finding the best split according to this saddle point objective will take exponential time. To make our approach practical and scalable, we propose efficient tree building algorithms by approximating the inner minimizer in this saddle point problem, and present efficient implementations for classical information gain based trees as well as state-of-the-art tree boosting models such as XGBoost. Experimental results on real world datasets demonstrate that the proposed algorithms can substantially improve the robustness of tree-based models against adversarial examples.

==> Oldstuff/old_toy_exp.tex <==
\subsection{Intuition and a Toy Example}
Regular training for a decision tree recursively chooses attributes and  setting thresholds by maximizing a given score, such as information gain. Note that there is an intrinsic consistency between the $\ell_\infty$ all and the decision boundary of a decision tree. So an easy approach for robust training is to maximize the minimum metric value obtained  the perturbation in an $\ell_\infty$ ball with radius $\epsilon$. A toy example with 10 points and 2 classes is shown in Figure~\ref{fig:pic0}.
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/example/Picture0.png}
  \caption{An toy example of training data}
  \label{fig:pic0}
\end{figure}
If we use the regular decision tree learning with maximum depth 1 and information gain as the metric, the optimal decision boundary is as shown in Figure~\ref{fig:pic1}. 
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/example/Picture1.png}
  \caption{Regular training, max depth=1, acc=0.8, worst acc=0}
  \label{fig:pic1}
\end{figure}
This split has information gain
\begin{equation}
\begin{split}
IG_{ori,reg}=&\frac{4}{10}\log(\frac{4/10}{1/2\cdot 1/2})+\frac{1}{10}\log(\frac{1/10}{1/2\cdot 1/2})\\+&\frac{4}{10}\log(\frac{4/10}{1/2\cdot 1/2})+\frac{1}{10}\log(\frac{1/10}{1/2\cdot 1/2})\\
&=0.278,
\end{split}
\end{equation} and the classification accuracy is 0.8. However, if an adversary is allowed to perturb the training data in an $\ell_\infty$ ball with radius 0.1, one possible perturbation as shown in Figure~\ref{fig:pic2} leads to an adversarial information gain as low as
\begin{equation}
\begin{split}
IG_{adv,reg}=&\frac{2}{10}\log(\frac{2/10}{1/2\cdot 1/2})+\frac{3}{10}\log(\frac{3/10}{1/2\cdot 1/2})\\+&\frac{2}{10}\log(\frac{2/10}{1/2\cdot 1/2})+\frac{3}{10}\log(\frac{3/10}{1/2\cdot 1/2})\\
&=0.029,
\end{split}
\end{equation}
and the classification accuracy is 0.6. The worst case accuracy is 0.
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/example/Picture2.png}
  \caption{Adversarial perturbation}
  \label{fig:pic2}
\end{figure}

A better decision boundary is as shown in Figure~\ref{fig:pic3}. With this decision boundary, within $\ell_\infty$ balls with radius 0.1, the information gain is always
\begin{equation}
\begin{split}
IG_{ori,rob}=IG_{adv,rob}=\frac{2}{10}\log(\frac{2/10}{1/2\cdot 2/10})\\+\frac{3}{10}\log(\frac{3/10}{1/2\cdot 8/10})+\frac{5}{10}\log(\frac{5/10}{1/2\cdot 8/10})=0.236,
\end{split}
\end{equation}
and the classification accuracy is always 0.7.
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/example/Picture3.png}
  \caption{Robust training, max depth=1, acc=0.7, worst acc=0.7}
  \label{fig:pic3}
\end{figure}

If the maximum tree depth is 2, the regular training will give a decision boundary as shown in Figure~\ref{fig:pic4} and he robust training will give a decision boundary as shown in Figure~\ref{fig:pic5}. If we use regular training, the accuracy on original data is 1, but at the worst case, the adversary can perturb the points to make accuracy 0.4. If we use robust training, the accuracy is guaranteed to be 0.7 in $\ell_\infty$ ball with radius 0.1.
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/example/Picture4.png}
  \caption{Regular training, max depth=2, acc=1, worst acc=0.4}
  \label{fig:pic4}
\end{figure}

\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/example/Picture5.png}
  \caption{Robust training, max depth=2, acc=0.7, worst acc=0.7}
  \label{fig:pic5}
\end{figure}


\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/example/RobustSplit.png}
  \caption{A split example with $M=6$, $N=6$, $m=4$, $n=2$, information gain 0.0817.}
  \label{fig:RobustSplit}
  \includegraphics[width=\linewidth]{Figures/example/AdvSplit.png}
  \caption{The split after adversarial perturbation. $M=6$, $N=6$, $m=3$, $n=3$, information gain 0.}
  \label{fig:AdvSplit}
\end{figure}

==> Oldstuff/oldstuff.tex <==
The greedy maximization step at each split is give by solving
$$k^*,\ \eta^*=\max_{\eta,k}S(k,\ \eta))$$
To obtain a robust split in an $\ell_\infty$ ball with radius $\epsilon$, We define the $robust\_score$ $RS(\eta,k)$ of a split $\eta$ on feature $k$ as
\begin{equation}
\begin{gathered}
    RS(\eta,k)\vcentcolon=\min_{I_L} S_I(I_L)\\
    \text{s.t. } I\cap\{(x_i,\ y_i)|x_i^k<\eta-\epsilon\}\subseteq I_L\subseteq I\cap\{(x_i,\ y_i)|x_i^k<\eta+\epsilon\}.
\end{gathered}
\label{eq:robust_score}
\end{equation}Maximizing $RS(\eta,k)$ is equivalent to solving a max-min problem 
\begin{equation}
\begin{gathered}
    \max_{\eta,k}\min_{I_L} S_I(I_L)\\
    \text{s.t. } I\cap\{(x_i,\ y_i)|x_i^k<\eta-\epsilon\}\subseteq I_L\subseteq I\cap\{(x_i,\ y_i)|x_i^k<\eta+\epsilon\}.
\end{gathered}
\label{eq:xgboost_max-min}
\end{equation}

In other words, splits of points in $$\Delta I(\eta,k,\epsilon)\vcentcolon=I\cap\{(x_i,\ y_i)|x_i^k\in[\eta-\epsilon,\eta+\epsilon)\}$$ are unsure.
Generally, this is a combinatorial optimization problem with complexity $O(2^{|\Delta I|})$. To solve this, we use a greedy approach. At each state, we calculate the score loss for each single possible adversarial perturbation and execute the perturbation with largest score loss. Also note that if for $\eta_1$ and $\eta_2$ we have $\Delta I(\eta_1,k,\epsilon)\subseteq\Delta I(\eta_2,k,\epsilon)$, we must have $RS(\eta_1,k)\geq RS(\eta_2,k)$. So we want to find $\eta$ with the smallest $\Delta I(\eta,k,\epsilon)$. To do this, it is sufficient to only consider $\Delta I=I\cap\{(x_i,\ y_i)|x_i^k\in[x_j^k-2\epsilon, x_j^k)\}$. The algorithm for robust split finding in XGBoost in shown in algorithm~\ref{alg:robust_xgboost_split}. The time complexity for a split is $O(dPn^2).$

\subsection{Approximate Optimal Solution for XGBoost}
For any point $j$ in $[\eta-\epsilon,\eta+\epsilon)$, we define $s_j\in\{0,1\}$ such that if $s_i=0$, we place point $i$ on the left and if $s_i=1$, we place point $i$ on the right. Let
$$G_1=\sum_{I_L\cap\{(x_i,\ y_i)|x_i^k<\eta+\epsilon\}}g_i,\ H_1=\sum_{I_L\cap\{(x_i,\ y_i)|x_i^k<\eta+\epsilon\}}h_i,$$
$$G_2=\sum_{I_L\cap\{(x_i,\ y_i)|x_i^k\geq\eta+\epsilon\}}g_i,\ H_2=\sum_{I_L\cap\{(x_i,\ y_i)|x_i^k\geq\eta+\epsilon\}}h_i.$$Then the minimization problem becomes
$$\min_{s_j\in\{0,1\}}\frac{(G_1-\sum_js_jg_j)^2}{H_1+\lambda-\sum_js_jh_j}+\frac{(G_2+\sum_js_jg_j)^2}{H_2+\lambda+\sum_js_jh_j},$$which is equivalent to
$$\min_{x,y}\frac{(G_1-x)^2}{H_1+\lambda-y}+\frac{(G_2+x)^2}{H_2+\lambda+y}\text{, such that } x=\sum_js_jg_j,\ y=\sum_js_jh_j.$$
Let $$f(x,y)=\frac{(G_1-x)^2}{H_1+\lambda-y}+\frac{(G_2+x)^2}{H_2+\lambda+y}$$(this function is \textbf{convex} when $0\leq y\leq H_1+\lambda$?) and we set
$$\frac{\partial f}{\partial x}=-\frac{2(G_1-x)}{H_1+\lambda-y}+\frac{2(G_2+x)}{H_2+\lambda+y}=0,$$
$$\frac{\partial f}{\partial y}=\frac{(G_1-x)^2}{(H_1+\lambda-y)^2}-\frac{(G_2+x)^2}{(H_2+\lambda+y)^2}=0.$$
We have when 
$$\frac{G_1-x}{H_1+\lambda-y}=\frac{G_2+x}{H_2+\lambda+y},$$
$\frac{\partial f}{\partial y}=\frac{\partial f}{\partial x}=0.$
We have $$(H_1+H_2+2\lambda)x-(G_1+G_2)y+[G_2(H_1+\lambda)-G_1(H_2+\lambda)]=0.$$
Note that we cannot use $\min_{x,y}f(x,y)$ as the lower bound. Because for any $G_1,\ G_2,\ H_1$ and $H_2$, we have $\min_{x,y}f(x,y)=\frac{(G_1+G_2)^2}{H_1+H_2+2\lambda}$ but $G_1+G_2$ and $H_1+H_2$ are constants with respect to any split. Then we approximate the optimal solution by finding $\{s_j\}$ which minimizes 
$$\min_{s_j}(\sum_jc_js_j-A)^2,$$
where $$c_j=(H_1+H_2+2\lambda)g_j-(G_1+G_2)h_j$$ and $$A=-G_2(H_1+\lambda)+G_1(H_2+\lambda).$$ This is equivalent to find the subset in $\{c_j\}$ whose sum is closest to $A$, which is a classical subset sum problem.  

\subsection{Robustness vs. Accuracy}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/accuracy_vs_robustness_lightbgm_untargeted.pdf}
  \caption{Robustness vs classification accuracy plot of LightGBM with with 255 bins and different numbers of trees.}
  \label{fig:robustness_vs_acc_lightgbm}
\end{figure}

\subsection{Robustness vs. Accuracy}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/accuracy_vs_robustness_lightbgm_untargeted_bin63.pdf}
  \caption{Robustness vs classification accuracy plot of LightGBM with 63 bins and different numbers of trees}
  \label{fig:robustness_vs_acc_lightgbm_bin63}
\end{figure}

\subsection{Robustness vs. Accuracy}
\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/accuracy_vs_robustness_lightbgm_untargeted_bin15.pdf}
  \caption{Robustness vs classification accuracy plot of LightGBM with 15 bins and different numbers of trees}
  \label{fig:robustness_vs_acc_lightgbm_bin15}
\end{figure}

\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/accuracy_vs_robustness_rf_untargeted.pdf}
  \caption{Robustness vs classification accuracy plot of Random Forest with different numbers of trees.}
  \label{fig:robustness_vs_acc_rf}
\end{figure}

\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/robustness_vs_accuracy_xgboost_higgs_l1.pdf}
\includegraphics[width=\linewidth]{Figures/robustness_vs_accuracy_xgboost_higgs_l2.pdf}
\includegraphics[width=\linewidth]{Figures/robustness_vs_accuracy_xgboost_higgs_linf.pdf}
  \caption{Robustness vs classification accuracy plot of XGBoost with different numbers of trees with HIGGS dataset }
  \label{fig:robustness_vs_acc_xgboost}
\end{figure}

\begin{figure}[ht]
  \includegraphics[width=\linewidth]{Figures/accuracy_vs_robustness_xgboost_con26.pdf}
  \caption{Robustness vs binary classification (2 vs. 6) accuracy plot of XGBoost with different numbers of trees. }
  \label{fig:robustness_vs_acc_xgboost_con26}
\end{figure}
